Momentum-Space Unitary Coupled Cluster and Translational Quantum Subspace Expansion for Periodic Systems on Quantum Computers

We demonstrate the use of the Variational Quantum Eigensolver (VQE) to simulate solid state crystalline materials. We adapt the Unitary Coupled Cluster ansatz to periodic boundary conditions in real space and momentum space representations and directly map complex cluster operators to a quantum circuit ansatz to take advantage of the reduced number of excitation operators and Hamiltonian terms due to momentum conservation. To further reduce required quantum resources, such as the number of UCCSD amplitudes, circuit depth, required number of qubits and number of measurement circuits, we investigate a translational Quantum Subspace Expansion method (TransQSE) for the localized representation of the periodic Hamiltonian. Additionally, we also demonstrate an extension of the point group symmetry based qubit tapering method to periodic systems. We compare accuracy and computational costs for a range of geometries for 1D chains of dimerized hydrogen, helium and lithium hydride with increasing number of momentum space grid points and also demonstrate VQE calculations for 2D and 3D hydrogen and helium lattices. Our presented strategies enable the use of near-term quantum hardware to perform solid state simulation with variational quantum algorithms.

==> tables/table_4.tex <==
\begingroup
\begin{table*}
     \caption{Comparison of energy values (in Ha) calculated with different methods on the periodic systems considered in this work. D stands for the number of dimensions in the periodic model.}
    \label{tab:energy_comparisons}
    \begin{ruledtabular}
    \begin{tabular}{lccc|ccc|ccc}
        & 
        $d$ ($\SI{}{\angstrom}$) &
        $D$ &
        $L$ & 
        $E_{\textrm{FCI}}^{\Gamma}/L$ & 
        $E_{\textrm{CCSD}}^{\Gamma}/L$ & 
        $E_{\textrm{UCCSD-PBC}}^{\Gamma}/L$ & 
        $E_{\textrm{UCCSD-PBC}}^{R}$ & 
        $E_{\textrm{UCCSD-PBC}}^{K}$ & 
        $E_{\textrm{TransQSE-W(2)}}$ 
        \\
        \hline
        H$_{2}$ & 
        $0.75$ &
        1 & 
        2 &
        $-1.0414576078$ & 
        $-1.0414491762$ & 
        $-1.0414573244$ & 
        $-1.0414573310$ &
        $-1.0414573245$ &
        --
        \\
        %H$_{2}$\footnote{Shot-based simulations, 8192 shots.} & 
        %$0.75$ &
        %1 & 
        %2 &
        % & 
        % & 
        % & 
        % &
        %xx &
        %--
        %\\ 
        H$_{2}$ & 
        $0.75$ &
        1 & 
        3 & 
        $-1.1232654641$ & 
        $-1.1231727367$ & 
        $-1.1231804970$ & 
        $-1.1231804857$ &
        $-1.1231804672$ &
        $-1.1175183195$
        \\ 
        H$_{2}$ & 
        $0.75$ &
        1 & 
        5 & 
        $-1.1051530344$ & 
        $-1.1050265451$ & 
        $-1.1050300023$ & 
        $-1.1050299871$ &
        $-1.1050299775$ &
        $-1.0945850884$ % -1.0945850921
        \\ 
        H$_{2}$ & 
        $0.75$ &
        1 & 
        9 & 
        -- & 
        $-1.1019109184$ & 
        -- & 
        -- &
        -- &
        $-1.0924256628$
        \\ 
        \hline               
        H$_{2}$ & 
        $0.75$ &
        2 & 
        4 & 
        $-1.0080293562$ & 
        $-1.0080185429$ & 
        $-1.0080274642$ & 
        -- &
        $-1.0080272592$ &
        --
        \\ 
        \hline               
        H$_{2}$\footnote{A  [2, 2] k-point mesh in the xy plane is selected for this calculation.} & 
        $0.75$ &
        3 & 
        4 & 
        $-1.2012791803$ & 
        $-1.2012520442$ & 
        $-1.2012684209$ & 
        -- &
        $-1.2012686107$ &
        --
        \\
        \hline
        He & 
        $1.0$ &
        1 & 
        2 &
        $-2.5285938200$ & 
        $-2.5285812803$ & 
        $-2.5285798759$ & 
        $-2.5285798742$ &
        $-2.5285798759$ &
        --
        \\ 
        He & 
        $1.0$ &
        1 & 
        3 & 
        $-2.7187307339$ & 
        $-2.7187230508$ & 
        $-2.7187216204$ & 
        $-2.7187266239$ &
        $-2.7187266447$ &
        $-2.7135013244$
        \\ 
        He & 
        $1.0$ &
        1 & 
        9 & 
        -- & 
        $-2.6848072550$ & 
        -- & 
        -- &
        -- &
        $-2.6749113551$
        \\ 
        \hline               
        He & 
        $1.0$ &
        2 & 
        4 & 
        $-2.2583587870$ & 
        $-2.2583498391$ & 
        $-2.2583476552$ & 
        -- &
        $-2.2583476554$ &
        --
        \\ 
        \hline               
        He$^{\text{a}}$ & 
        $1.0$ &
        3 & 
        4 & 
        $-2.9562190137$ & 
        $-2.9562164816$ & 
        $-2.9562162171$ & 
        -- &
        $-2.9562162173$ &
        --
        \\
        \hline               
        LiH & 
        $2.0$ &
        1 & 
        3 & 
        $-7.9828384941$ & 
        $-7.9824545358$ & 
        $-7.9825328540$ & 
        $-7.9825334480$ &
        $-7.9825334389$ &
        --
        \\
    \end{tabular}
    \end{ruledtabular}

\end{table*}
\endgroup
